Why we couldn't prove SETH hardness of the Closest Vector Problem for even norms!

Recent work [BGS17,ABGS19] has shown SETH hardness of CVP in the $\ell_p$ norm for any $p$ that is not an even integer. This result was shown by giving a Karp reduction from $k$-SAT on $n$ variables to CVP on a lattice of rank $n$. In this work, we show a barrier towards proving a similar result for CVP in the $\ell_p$ norm where $p$ is an even integer. We show that for any $c>0$, if for every $k > 0$, there exists an efficient reduction that maps a $k$-SAT instance on $n$ variables to a CVP instance for a lattice of rank at most $n^{c}$ in the Euclidean norm, then $\mathsf{coNP} \subset \mathsf{NP/Poly}$. We prove a similar result for CVP for all even norms under a mild additional promise that the ratio of the distance of the target from the lattice and the shortest non-zero vector in the lattice is bounded by $exp(n^{O(1)})$. Furthermore, we show that for any $c> 0$, and any even integer $p$, if for every $k > 0$, there exists an efficient reduction that maps a $k$-SAT instance on $n$ variables to a $SVP_p$ instance for a lattice of rank at most $n^{c}$, then $\mathsf{coNP} \subset \mathsf{NP/Poly}$. The result for SVP does not require any additional promise. While prior results have indicated that lattice problems in the $\ell_2$ norm (Euclidean norm) are easier than lattice problems in other norms, this is the first result that shows a separation between these problems. We achieve this by using a result by Dell and van Melkebeek [JACM, 2014] on the impossibility of the existence of a reduction that compresses an arbitrary $k$-SAT instance into a string of length $\mathcal{O}(n^{k-\epsilon})$ for any $\epsilon>0$. In addition to CVP, we also show that the same result holds for the Subset-Sum problem using similar techniques.

==> extra.tex <==

\section{Reducing Exact-SVP to Approx-SVP}
\begin{lemma}\cite{AD16}[Lemma~2]\label{lem:SVP-coeff-bound}
Let $\basis=[\vect{b}_1,\vect{b}_2,\cdots , \vect{b}_n]$ be a LLL-reduced basis and $\vect{u}=\sum\limits_{i=1}^n \alpha_i\vect{b}_i$ be a shortest vector of the lattice. Then, for all $i\in [n], |\alpha_i|\leq 2^{3(n-1)/2}$. 
\end{lemma}


\begin{theorem}
There is a polynomial time reduction from $\SVP$ to $(1+\epsilon)$-$\SVP$ where $\epsilon=2^{-\mathcal{O}(n^2)}$.
\end{theorem}

\begin{proof}
Let $\SVP(\basis,d)$ be the given instance where $\basis\in \intg^{m\times n}$ and $d>0$ is a number. We can assume that basis $\basis$ is a LLL-reduced basis. From LLL algorithm, we also get a number $D>0$ satisfying $\lambda_1(\cL(\basis))\leq D\leq 2^{n/2}\lambda_1(\cL(\basis))$. Let for all $i\in [n]$, $\epsilon_i=\frac{2^{2(i-1)n}}{2^{2n^2}}D$. Let 
\[\basis'=\begin{bmatrix} \vect{b}_1' & \vect{b}_2' & \cdots & \vect{b}_n' \end{bmatrix}=\begin{bmatrix}\vect{b}_1 & \vect{b}_2& \cdots & \vect{b}_n \\
\epsilon_1 & 0 &\cdots & 0\\
0 & \epsilon_2 & \cdots & 0\\
\vdots & \vdots & \vdots & \vdots \\
0 & 0 & \cdots & \epsilon_n
\end{bmatrix}.\]
Let $\cL'$ be the lattice generated by basis $\basis'$. It is easy to see that $\lambda_1(\cL)< \lambda_1(\cL')$. Let $\vect{u}=\sum\limits_{i=1}^n \alpha_i\vect{b}_i$ be a shortest vector of lattice $\cL$. From Lemma~\ref{lem:SVP-coeff-bound}, we know that for all $i\in [n], |\alpha_i|\leq 2^{3(n-1)/2}$. Let $\vect{v}=\sum\limits_{i=1}^n \alpha_i\vect{b}_i'\in \cL'$, we get 
\begin{align*}
    \|\vect{v}\|^2=\|\vect{u}\|^2+\sum\limits_{i=1}^n \alpha_i^2\epsilon_i^2 & \leq \lambda_1^2(\cL)+2^{3(n-1)}D^2\sum\limits_{i=1}^n \frac{2^{4(i-1)n}}{2^{4n^2}} \\
    & \leq \lambda_1^2(\cL)+2^{3(n-1)}D^2\frac{2^{4n^2}-1}{2^{4n^2}(2^{4n}-1)} \\
    & \leq \lambda_1^2(\cL)+ 2^{-n}D^2 \leq 2\lambda_1^2(\cL). 
\end{align*}
Hence, $\lambda_1(\cL')\leq \sqrt{2}\cdot\lambda_1(\cL)$. Let $\vect{u}_1=\sum\limits_{i=1}^n x_i\vect{b}_i$ and $\vect{u}_2=\sum\limits_{i=1}^n y_i\vect{b}_i$ be two distinct vectors of length $\lambda_1(\cL)$ in lattice $\cL$. Let $k\in [n]$ be the largest index such that $x_k\neq y_k$. Let $\vect{v}_1=\sum\limits_{i=1}^n x_i\vect{b}_i'$ and $\vect{v}_2=\sum\limits_{i=1}^n y_i\vect{b}_i'$, then 
\begin{align*}
\left|\|\vect{v}_1\|^2-\|\vect{v}_2\|^2\right|\leq \left|\sum\limits_{i=1}^n |x_i^2-y_i^2| \epsilon_i^2\right| &\leq \epsilon_k^2- 2^{3n-2)}D^2 \sum\limits_{i=1}^{k-1} \frac{2^{4(i-1)n}}{2^{4n^2}} \\
& \leq D^2\left(\frac{2^{4(k-1)n}}{2^{4n^2}} - 2^{3n-2}\frac{2^{4(k-1)n}-1}{2^{4n^2}(2^{4n}-1)}\right)\\
&\leq 2^{-4n^2} \cdot D^2.
\end{align*}

Therefore it is a $\gamma$-$u\SVP$ instance, where 
\color{red}
\begin{align*}
    \gamma=\left(\frac{\lambda_2^2(\cL')}{\lambda_1^2(\cL')}\right)^{1/2} \geq \left(\frac{\lambda_1^2(\cL')+2^{-4n^2}D^2}{\lambda_1^2(\cL')} \right)^{1/2} &\geq \left(\frac{2\lambda_1^2(\cL)+2^{-4n^2}D^2}{2\lambda_1^2(\cL)} \right)^{1/2}\\
    & \geq \left(1+\frac{2^{-4n^2 \lambda_1^2(\cL)}}{2\lambda_1^2(\cL)}\right)^{1/2}\\
    & \geq 1+2^{-4n^2-3}.
\end{align*} 
\color{black}
The $\lambda_2(\cL')$ can be smaller than $(\lambda_1^2(\cL')+2^{-4n^2}D^2)^{1/2}$. It can be something like $\lambda_1(\cL)+1$.
\end{proof}


\section{Reducing Exact-CVP to Approx-CVP}

\begin{theorem}
There is a polynomial time reduction from $\CVP$ to $(1+\epsilon)$-$\CVP$ where $\epsilon=2^{-\mathcal{O}(n^3)}$.
\end{theorem}

\begin{proof}
Let $\CVP(\basis,\vect{t},d)$ be the given instance where $\basis\in \intg^{m\times n}$, target $\vect{t}\in \intg^{m}$ and $d>0$ is a number. From Lemma~\ref{lem:dimension-reduction}, we can assume that $m=n+1$. By Proposition~\ref{prop:coeff-bound}, we can assume that for all $\vect{z}\in \intg^n$ for which $\|\mathbf{B}\vect{z}-\vect{t}\|=\dist(\mathbf{B},\vect{t})$ satisfies  $\|\vect{z}\|_\infty < 2^{10n^2}$. From Babai's CVP algorithm, we get a number $D>0$ satisfying $\dist(\cL(\basis),\vect{t})\leq D\leq 2^{n/2}\dist(\cL(\basis),\vect{t})$. Let for all $i\in [n]$, $\epsilon_i=\frac{2^{11(i-1)n^2}}{2^{11n^3}}D$. Let 
\[\basis'=\begin{bmatrix} \vect{b}_1' & \vect{b}_2' & \cdots & \vect{b}_n' \end{bmatrix}=\begin{bmatrix}\vect{b}_1 & \vect{b}_2& \cdots & \vect{b}_n \\
\epsilon_1 & 0 &\cdots & 0\\
0 & \epsilon_2 & \cdots & 0\\
\vdots & \vdots & \vdots & \vdots \\
0 & 0 & \cdots & \epsilon_n
\end{bmatrix} \text{ and } \vect{t}'=\begin{bmatrix}\vect{t}\\ 0 \\ 0 \\ \vdots \\ 0\end{bmatrix} .\]
Let $\cL'$ be the lattice generated by basis $\basis'$. It is easy to see that $\dist(\cL,\vect{t})< \dist(\cL',\vect{t}')$. Let $\vect{u}=\sum\limits_{i=1}^n \alpha_i\vect{b}_i$ be a closet lattice vector in $\cL$  vector to target vector $\vect{t}$.  We know that for all $i\in [n], |\alpha_i|\leq 2^{10n^2}$. Let $\vect{v}=\sum\limits_{i=1}^n \alpha_i\vect{b}_i'\in \cL'$, we get 
\begin{align*}
    \|\vect{v}-\vect{t}'\|^2=\|\vect{u}-\vect{t}\|^2+\sum\limits_{i=1}^n \alpha_i^2\epsilon_i^2 & \leq \dist^2(\cL,\vect{t})+2^{20n^2}D^2\sum\limits_{i=1}^n \frac{2^{22(i-1)n^2}}{2^{22n^3}} \\
    & \leq \dist^2(\cL,\vect{t})+2^{20n^2}D^2\frac{2^{22n^3}-1}{2^{22n^3}(2^{22n^2}-1)} \\
    & \leq \lambda_1^2(\cL)+ 2^{-20n^2}D^2 \leq 2\cdot\dist^2(\cL,\vect{t}). 
\end{align*}
Hence, $\dist(\cL',\vect{t}')\leq \sqrt{2}\cdot\dist(\cL,\vect{t})$. Let $\vect{u}_1=\sum\limits_{i=1}^n x_i\vect{b}_i$ and $\vect{u}_2=\sum\limits_{i=1}^n y_i\vect{b}_i$ be two distinct lattice whose distance from $\vect{t}$ is $\dist(\cL,\vect{t})$. Let $k\in [n]$ be the largest index such that $x_k\neq y_k$. Let $\vect{v}_1=\sum\limits_{i=1}^n x_i\vect{b}_i'$ and $\vect{v}_2=\sum\limits_{i=1}^n y_i\vect{b}_i'$, then 
\begin{align*}
\left|\|\vect{v}_1\|^2-\|\vect{v}_2\|^2\right|\leq \left|\sum\limits_{i=1}^n |x_i^2-y_i^2| \epsilon_i^2\right| &\leq \epsilon_k^2- 2^{20n^2}D^2 \sum\limits_{i=1}^{k-1} \frac{2^{22(i-1)n^2}}{2^{22n^3}} \\
& \leq D^2\left(\frac{2^{22(k-1)n^2}}{2^{22n^3}} - 2^{20n^2}\cdot\frac{2^{22(k-1)n^2}-1}{2^{22n^3}(2^{22n^2}-1)}\right)\\
&\leq 2^{-22n^3} \cdot D^2.
\end{align*}

It implies that there is only a unique lattice vector in $\cL'$ whose length from target vector $\vect{t'}$ is less than $\left(\dist(\cL',\vect{t}')^2+2^{-22n^3}\cdot D^2\right)^{1/2}$. By using the bound on $D$, we get 

\begin{align*}
    \frac{\dist^2(\cL',\vect{t}')+2^{-22n^3}\cdot D^2}{\dist^2(\cL',\vect{t}')} &\geq \frac{\dist^2(\cL',\vect{t}')+2^{-22n^3}\cdot \dist^2(\cL,\vect{t})}{\dist^2(\cL',\vect{t}')}\\
    & \geq \frac{2\cdot\dist^2(\cL,\vect{t})+2^{-22n^3}\cdot \dist^2(\cL,\vect{t})}{2\cdot\dist^2(\cL,\vect{t})}\\
    & \geq 1+2^{-22n^3-1}.
\end{align*}

Hence,     



\end{proof}


==> instance-compress-subset-sum.tex <==
\section{Proof of \cref{lem:compress-subset-sum}}

\begin{proof}
We are given a set of integers $a_1,\cdots, a_n$ and the target integer $t$ where $|a_i|,|t|\leq 2^{\eta}$. The goal is to distinguish whether there exist a subset of numbers whose sum is equal to $t$ or not. 

Our instance compression algorithm will reduce this problem to the modular \textsf{Subset-Sum} problem where given integers $a_1',\ldots, a_n',$ target $t'$, and modulus $p$, the task is to decide whether there exists a subset of the $a_i'$ such that their sum is equal to $t'$ modulo $p$. 

The algorithm samples a uniformly random prime number $p$ from $[2^{10n+2\log \eta+10},2^{20n+2\log \eta+10}]$. Let $ a_i'=a_i\mod p $ for all $i \in [n]$, and $t'=t\mod p $. Since $a_i'$ and $t'$ are numbers modulo $p \le 2^{20n+2\log \eta+10}$, we can store all of them as a bitstring of length $O(n^2+n\log \eta))$. In the rest of the proof, we will show the correctness of the reduction..

If the given \textsf{Subset-Sum} instance is a \textsf{YES} instance, then there exists a $\vect{z}\in \{0,1\}^n$ such that $\sum_{i=1}^n z_ia_i=t$. This implies that $\sum_{i=1}^n z_ia_i'\mod p=t\mod p = t' \mod p$. Thus, the resulting instance is a \textsf{YES} instance of the modular \textsf{Subset-Sum} problem. Notice that, we don't get any error in this case.

Now, let's assume that for all $\vect{z}\in \{0,1\}^n$, $\sum_{i=1}^n z_i a_i\neq t$ \textit{i.e.} given \textsf{Subset-Sum} instance is a \textsf{NO} instance. Now we will show that, with overwhelming probability, for all $\vect{z}\in \{0,1\}^n$, $\sum_{i=1}^n z_i a_i'\neq t'\mod p$. From an extension of the prime number theorem~\cite{HB88} we know that number of primes in range $[2^{10n+2\log \eta+10}, 2^{20n+2\log \eta+10}]$ is at least
\[\frac{2^{20n+2\log \eta+9}}{20n+2\log \eta+10} \ge 2^{20n+\log \eta} \;.\]
Also, for any fixed $\vect{z}\in \{0,1\}^n$, $|\sum_{i=1}^n z_ia_i-t| \le (n+1)\cdot 2^\eta$, and hence, there are at most 
\[
\log(2^\eta \cdot (n+1)) = \eta + \log (n+1)
\]
distinct primes  that divide $\sum_{i=1}^n z_ia_i-t$. Hence, with probability, at most
\[
\frac{\eta+\log(n+1)}{2^{20 n + \log \eta}} \le 2^{-19n}\;,
\]
the prime $p$ is such that
 $\sum_{i=1}^n z_ia_i-t = 0\mod p$. By applying a union bound, we get that
\[\Pr\left[\exists \vect{z}\in \{0,1\}^n,\sum_{i=1}^n z_ia_i-t\mod p= 0 \right] \leq {2^{-19n}}\cdot 2^{n} \leq 2^{-18n} .\]
This implies that, with at least $1-2^{-18n}$ probability, there exists no vector $\vect{z}\in \{0,1\}^n$, such that $(\sum z_ia_i-t)\mod p= (\sum z_ia_i'-t')\mod p$ is non-zero in $\mathbb{Z}_p$. This completes the proof. 
\end{proof}

